Distributed Indirect Source Coding with Decoder Side Information

This paper studies a variant of the rate-distortion problem motivated by task-oriented semantic communication and distributed learning problems, where $M$ correlated sources are independently encoded for a central decoder. The decoder has access to a correlated side information in addition to the messages received from the encoders, and aims to recover a latent random variable correlated with the sources observed by the encoders within a given distortion constraint rather than recovering the sources themselves. We provide bounds on the rate-distortion region for this scenario in general, and characterize the rate-distortion function exactly when the sources are conditionally independent given the side information.

==> old/name.tex <==
%\documentclass[conference, onecolumn]{IEEEtran}
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{makecell}
\usepackage{verbatim}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\begin{document}

\title{Distributed Compression of Semantic Information with Decoder Side Information\\

%\thanks{Identify applicable funding agency here. If none, delete this.}
}



    

\maketitle

\begin{abstract}
This paper study a variant rate distortion problem motivated by goal-oriented semantic communication. The semantic information source corresponding to the task consists of a set of correlated random variables whose joint probabilistic distribution can be described by a Bayesian network. We consider a 5-variables semantic source where only three variables need to be separately encoded in a lossy fashion and the rest two variables are revealed to the decoder as side information. We establish bounds on the rate-distortion region for this scenario and derive a conclusive rate-distortion function when the three variables are conditionally independent given the side information.

\begin{IEEEkeywords} Semantic communication, rate distortion, semantic compression.
\end{IEEEkeywords}
\end{abstract}




\section{Introduce}
Shannon's classical information theory, established in 1948, forms the foundation of modern communication systems. Focusing on symbol transmission and disregarding semantic content, Shannon introduced information entropy based on symbol probability to quantitatively measure the size of information \cite{b1}. This framework gives theoretical boundaries for source compression and data transmission. Over the last 70 years, advancements like polar codes and multiple-input multiple-output (MIMO) systems have brought current communication systems close to Shannon's capacity \cite{b2} \cite{b3}. Semantic or Task-oriented communication based on Deep Learning has been viewed as a promising to break through the Shannon limits due to its outstanding effectiveness. 


In recent years, there has been some progress in the study of semantic information theory. Photis \emph{et al.} introduced a novel source model where the semantic information is considered as an inherent part of the source. In this model, the semantic information is not directly observable but can be deduced from the extrinsic state \cite{Photios1,Photios2,Photios3}. Similarly, Guo et al. determined the theoretical boundaries for the semantic rate distortion problem with side information based on the indirect semantic source model \cite{Guo}. In \cite{Concepts}, the authors considered the problem of communicating a sequence of unknown and potentially stochastic maps, and provided a bound for the distortion-rate function.

Despite various efforts, a general and well accepted theory of semantic information remains elusive, and fundamental limits essential for guiding the design of semantic communication systems are yet to be established. Consequently, there is an urgent need to formulate a mathematical theory of semantic communication to address these foundational issues.

In this paper, the semantic information source is modelled as a set of correlated semantic elements whose joint distribution can be represent by a Bayesian network (BN). We investigate the lossy compression problem with the 5-variables semantic source as illustrated in Fig.~\ref{system}, where three dependent discrete variables $X_1, X_2, X_3$ need to be encoded separately, and the decoder is allowed to observe the side information stream generated by the discrete variables $Z, F$. The conditional dependence relations among the variables are shown in Fig.~\ref{bn}. Slepian and Wolf \cite{slepian} have studied the scenario where only $X_1$ and  $X_2$ need to be encoded separately in a lossless fashion, but decoded together without side information. Their result reveal that the total rate required for individual (lossless) compression of $X_1$ and $X_2$ is equivalent to the rate required for compressing $X_1$ and $X_2$ jointly. Wyner and Ziv \cite{wyner1, wyner2} have studied the lossy compression of a single source $X_1$ with side information at decoder. They determined the rate-distortion function for this case. Michael \cite{Michael} considered the  lossy compression scenario where $X_1$ and $X_2$  are compressed separately  and the decoder  has access to side information $Z$. They provided conclusive rate-distortion results for the special case where $X_1$ and $X_2$ are conditionally independent given the side information $Z$.
\begin{figure}
\centerline{\includegraphics[width=1in]{fig/Graph.png}}
\caption{The conditional dependence relations among $X_1, X_2, X_3, Z, F$.}
\label{bn}
\end{figure}

\begin{figure}
\centerline{\includegraphics[width=2in]{fig/System.png}}
\caption{Separate compression of three sources with side information at receiver.}
\label{system}
\end{figure}


In the problem studied in this paper, we aim to derive a rate distortion region, denoted as $R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}} \right)$, which is defined as the set of rate triples $(R_1, R_2, R_3)$ that permit the expected distortion to meet the distortion constrains

\begin{equation}
\begin{aligned}
E{d_1}({X_1},{\hat X_1}) \leqslant {D_1},\\
E{d_2}({X_2},{\hat X_2}) \leqslant {D_2},\\
E{d_3}({X_3},{\hat X_3}) \leqslant {D_3},
\end{aligned}
\label{constrains}
\end{equation}
where the distortion measure $d_i$ is arbitrary, and $\hat X_i$ the estimate of $X_i$  given the received codeword indices and the side information. All of the variables $X_1, X_2, X_3, Z, F$ take values in finite sets  $\mathcal{X}_1, \mathcal{X}_2, \mathcal{X}_3, \mathcal{Z}$ and  $\mathcal{F}$. Their joint distribution $p\left( {{x_1},{x_2},{x_3},z,f} \right)$ is given.


%In this paper, we study the Wyner-Ziv problem with three discrete memoryless dependent sources $X_1$, $X_2$, $X_3$ and two side information random variable $Z$, $F$,  whose  causal relationships are modeled by a Bayesian Network as shown in Fig.~\ref{bn}. Their joint distribution $p\left( {{x_1},{x_2},{x_3},z,f} \right)$ is given. 

In section II, we derive an achievable region $R_a\left( {{D_1},{D_2}, {D_3}} \right) \subseteq R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$.
In section III, we determine a general outer bound $R_o\left( {{D_1},{D_2}, {D_3}} \right)  \supseteq  R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$.
In section IV, we show that the two regions coincide and the region is optimal under the scenario as shown in Fig.~\ref{bn}. %when the three source are conditionally independent given the side information.


\section{An Achievable Rate Region}

In this section, we derive an achievable rate region $R_a\left( {{D_1},{D_2}, {D_3}} \right) $ which is contained by the goal rate-distortion region $R_a\left( {{D_1},{D_2}, {D_3}} \right) \subseteq R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$.

\textbf{Lemma 1 (extended Markov lemma)} Let
\begin{equation}
\begin{aligned}
&p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) \\&= p\left( {{w_1}|{x_1}} \right)p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right) p\left( {{x_1},{x_2},{x_3},z,f} \right).
\end{aligned}
\label{extend mk}
\end{equation}
For a fixed $\left( {{x_1^n},{x_2^n},{x_3^n},z^n, f^n} \right) \in A_\epsilon^{*\left( n \right)}$, $W_1^n$ is drown from $p(w_1|x_1)$, which implies that $(x_1^n, W_1^n)  \in A_\epsilon^{*\left( n \right)} $ for sufficiently large $n$. $W_2^n$ is drown from $p(w_2|x_2)$, which implies that $(x_2^n, W_2^n)  \in A_\epsilon^{*\left( n \right)} $ for sufficiently large $n$, $W_3^n$ is drown from $p(w_3|x_3)$, which implies that $(x_3^n, W_3^n)  \in A_\epsilon^{*\left( n \right)} $ for sufficiently large $n$. Then with high probability, $\left( {W_1^n,W_2^n,W_3^n,{x_1^n},{x_2^n},{x_3^n},z^n, f^n} \right) \in A_\epsilon^{*\left( n \right)}$.

\emph{Proof:} According to \eqref{extend mk}, we have several Markov chains  $W_1-X_1-(X_2,X_3,Z,F)$, $W_2-X_2-(X_1,X_2,Z,F)$, $W_3-X_3-(X_1,X_2,Z,F)$, $W_1-(X_1,X_2,X_3,Z,F)-W_2$, $W_1-(X_1,X_2,X_3,Z,F)-W_3$, $W_2-(X_1,X_2,X_3,Z,F)-W_3$. We use the Markov lemma three times, first to derive that $((x_2^n,x_3^n,z^n,f^n),x_1^n,w_1^n)$ are jointly typical, $((x_1^n,x_3^n,z^n,f^n),x_2^n,w_2^n)$ are jointly typical and $((x_1^n,x_2^n,z^n,f^n),x_3^n,w_3^n)$ are jointly typical. Then using the relationships $W_3-X_3-(X_1,X_2,Z,F)$, $W_1-(X_1,X_2,X_3,Z,F)-W_2$, $W_1-(X_1,X_2,X_3,Z,F)-W_3$, $W_2-(X_1,X_2,X_3,Z,F)-W_3$, we can demonstrate that $\left( {w_1^n,w_2^n,w_3^n,{x_1^n},{x_2^n},{x_3^n},z^n, f^n} \right)$ are joint typical.





\textbf{Theorem 2:} $R_a\left( {{D_1},{D_2}, {D_3}} \right) \subseteq R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$, where $R_a\left( {{D_1},{D_2}, {D_3}} \right)$ is the set of all rate triples $(R_1,R_2,R_3)$ such that there exists a triple  $(W_1,W_2,W_3)$ of discrete random variables with $p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_1}|{x_1}} \right)$$p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right)$ $ p\left( {{x_1},{x_2},{x_3},z,f} \right)$ for which the following conditions are satisfied

\begin{equation*}
\begin{footnotesize}
\begin{aligned}
  {R_1} &\geqslant I\left( {{X_1};{W_1}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right) \hfill \\
  {R_2} &\geqslant I\left( {{X_2};{W_2}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \hfill \\
  {R_3} &\geqslant I\left( {{X_3};{W_3}} \right) - I\left( {{W_3};{W_1},{W_2},Z,F} \right) \hfill \\
\end{aligned}
\label{achieve region}
\end{footnotesize}
\end{equation*}
\begin{equation*}
\begin{footnotesize}
\begin{aligned}
  {R_1} + {R_2} &\geqslant I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\&- I\left( {{W_2};{W_1},{W_3},Z,F} \right) + I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \hfill \\
  {R_1} + {R_3} &\geqslant I\left( {{X_1};{W_1}} \right) + I\left( {{X_3};{W_3}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_1};{W_3}|{W_2},Z,F} \right) \hfill \\
 {R_2} + {R_3} &\geqslant I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_2};{W_3}|{W_1},Z,F} \right) \hfill \\
\end{aligned}
\label{achieve region}
\end{footnotesize}
\end{equation*}
\begin{equation}
\begin{footnotesize}
\begin{aligned}
 {R_1} + {R_2} + {R_3} &\geqslant I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) \\&- I\left( {{W_1};{W_2},{W_3},Z,F} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \\&+ I\left( {{W_1},{W_2};{W_3}|Z,F} \right),
 \hfill \\ 
\end{aligned}
\label{achieve region}
\end{footnotesize}
\end{equation}
and for which there exist decoding functions ${g_1}\left(  \cdot  \right)$, ${g_2}\left(  \cdot  \right)$ and ${g_3}\left(  \cdot  \right)$ such that

\begin{equation}
\begin{aligned}
E{d_1}({X_1},{g_1(W_1,W_2,W_3,Z,F)}) \leqslant {D_1},\\
E{d_2}({X_2},{g_2(W_2,W_1,W_3,Z,F)}) \leqslant {D_2},\\
E{d_3}({X_3},{g_3(W_3,W_1,W_2,Z,F)}) \leqslant {D_3},
\end{aligned}
\label{constrains}
\end{equation}

The rigorous proof of Theorem 2 is provided in Appendix A.



\section{An General Outer Bound}

In this section, we derive a region $R_o\left( {{D_1},{D_2}, {D_3}} \right) $ which contains the goal rate-distortion region $R_o\left( {{D_1},{D_2}, {D_3}} \right)  \supseteq  R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$.

\textbf{Theorem 3:} $R_o\left( {{D_1},{D_2}, {D_3}} \right)  \supseteq  R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$, where $R_o\left( {{D_1},{D_2}, {D_3}} \right) $ is the set of all rate triples $(R_1,R_2,R_3)$ such that there exists a triple  $(W_1,W_2,W_3)$ of discrete random variables with  $p\left( {{w_1}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_1}|{x_1}} \right)$, $p\left( {{w_2}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_2}|{x_2}} \right)$ and $p\left( {{w_3}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_3}|{x_3}} \right)$ for which the following conditions are satisfied

\begin{equation*}
\begin{footnotesize}
\begin{aligned}
{R_1} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right) \\&= I\left( {{W_1};{X_1}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right)\\
{R_2} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F} \right) \\&= I\left( {{W_2};{X_2}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right)\\
{R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_3}|{W_1},{W_2},Z,F} \right) \\&= I\left( {{W_3};{X_3}} \right) - I\left( {{W_3};{W_1},{W_2},Z,F} \right)\\
\end{aligned}
\end{footnotesize}
\end{equation*}
\begin{equation*}
\begin{footnotesize}
\begin{aligned}
{R_1} + {R_2} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1},{W_2}|{W_3},Z,F} \right) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\&- I\left( {{W_2};{W_1},{W_3},Z,F} \right) + I\left( {{W_1};{W_2}|{W_3},Z,F} \right)\\
{R_1} + {R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1},{W_3}|{W_2},Z,F} \right) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_3};{W_3}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right)\\& - I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_1};{W_3}|{W_2},Z,F} \right)\\
{R_2} + {R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_2},{W_3}|{W_1},Z,F} \right) \\&= I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_2};{W_3}|{W_1},Z,F} \right)\\
\end{aligned}
\end{footnotesize}
\end{equation*}
\begin{equation}
\begin{footnotesize}
\begin{aligned}
{R_1} + {R_2} + {R_3} &\geqslant I(X_1, X_2, X_3; W_1, W_2, W_3| Z, F) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) \\&- I\left( {{W_1};{W_2},{W_3},Z,F} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \\&+ I\left( {{W_1},{W_2};{W_3}|Z,F} \right),
\end{aligned}
\end{footnotesize}
\label{theorem3}
\end{equation}
and for which there exist decoding functions ${g_1}\left(  \cdot  \right)$, ${g_2}\left(  \cdot  \right)$ and ${g_3}\left(  \cdot  \right)$ such that

\begin{equation}
\begin{aligned}
E{d_1}({X_1},{g_1(W_1,W_2,W_3,Z,F)}) \leqslant {D_1},\\
E{d_2}({X_2},{g_2(W_2,W_1,W_3,Z,F)}) \leqslant {D_2},\\
E{d_3}({X_3},{g_3(W_3,W_1,W_2,Z,F)}) \leqslant {D_3},
\end{aligned}
\label{constrains}
\end{equation}

The rigorous proof of Theorem 3 is provided in Appendix B.



%According to the joint distribution $p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_1}|{x_1}} \right)p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right)$ $ p\left( {{x_1},{x_2},{x_3},z,f} \right)$, we have several Markov chains: $W_1-(X_1,X_2,X_3,Z,F)-W_2$, $W_1-(X_1,X_2,X_3,Z,F)-W_3$, $W_2-(X_1,X_2,X_3,Z,F)-W_2$, $W_1-X_1-(X_2,X_3,Z,F)$, $W_2-X_2-(X_1,X_2,Z,F)$, $W_3-X_3-(X_1,X_2,Z,F)$.




\section{conclusive rate-distortion results}

\emph{Corollary 4:} If the joint distribution of $X_1, X_2, X_3, Z, F$ can be modelled by the BN as shown in Fig.~\ref{bn}, $R_a\left( {{D_1},{D_2}, {D_3}} \right) \subseteq R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$ where $R_a\left( {{D_1},{D_2}, {D_3}} \right) $ is the set of all rate triples $(R_1,R_2,R_3)$ such that there exists a triple $(W_1,W_2,W_3)$ of discrete random variables with $p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_1}|{x_1}} \right)p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right)p\left( {{x_1}|z} \right) p\left( {{x_2}|z} \right) p\left( {{z}|f} \right) p\left( {{x_3}|f} \right)$ $ p\left( {f} \right)$ for which the following conditions are satisfied

\begin{equation}
\begin{aligned}
  {R_1} &\geqslant I\left( {{X_1};{W_1}} \right) - I\left( {{W_1};Z,F} \right) \hfill \\
  {R_2} &\geqslant I\left( {{X_2};{W_2}} \right) - I\left( {{W_2};Z,F} \right) \hfill \\
  {R_3} &\geqslant I\left( {{X_3};{W_3}} \right) - I\left( {{W_3};Z,F} \right) \hfill \\
\end{aligned}
\label{achieve region}
\end{equation}

and for which there exist decoding functions ${g_1}\left(  \cdot  \right)$, ${g_2}\left(  \cdot  \right)$ and ${g_3}\left(  \cdot  \right)$ such that

\begin{equation}
\begin{aligned}
E{d_1}({X_1},{g_1(W_1,W_2,W_3,Z,F)}) \leqslant {D_1},\\
E{d_2}({X_2},{g_2(W_2,W_1,W_3,Z,F)}) \leqslant {D_2},\\
E{d_3}({X_3},{g_3(W_3,W_1,W_2,Z,F)}) \leqslant {D_3},
\end{aligned}
\label{constrains}
\end{equation}

\emph{Proof.} Since the joint distribution can be written as 
\begin{equation}
\begin{aligned}
&p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) \\&= p\left( {{w_1}|{x_1}} \right)p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right)p\left( {{x_1}|z} \right) p\left( {{x_2}|z} \right)\\& \times p\left( {{z}|f} \right) p\left( {{x_3}|f} \right)p\left( {f} \right).
\end{aligned}
\end{equation}
The terms in the sum rate bound \eqref{achieve region} $I\left( {{W_1};{W_2}|{W_3},Z,F}\right)$, $ I\left( {{W_1};{W_3}|{W_2},Z,F}\right)$ and $I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_2};{W_3}|{W_1},Z,F}\right)$ are zero. Therefore, the sum rate bound can be expressed as the sum of the side bounds and can be omitted. The side bounds in \eqref{achieve region} can be written as
\begin{equation}
\begin{footnotesize}
\begin{aligned}
I\left( {{W_1};{W_2},{W_3},Z,F} \right) = I\left( {{W_1};Z,F} \right) + I\left( {{W_2},{W_3};{W_1}|Z,F} \right) \\
I\left( {{W_2};{W_1},{W_3},Z,F} \right) = I\left( {{W_2};Z,F} \right) + I\left( {{W_1},{W_3};{W_2}|Z,F} \right) \\
I\left( {{W_3};{W_1},{W_2},Z,F} \right) = I\left( {{W_3};Z,F} \right) + I\left( {{W_1},{W_2};{W_3}|Z,F} \right),
\end{aligned}  
\end{footnotesize}
\end{equation}
where the last terms in the right hand side are 0. This proves the corollary 4.

%A Bayesian network is a mathematical model for representing causal relationships among random variables by using conditional probabilities.

\emph{Corollary 5:} If the joint distribution of $X_1, X_2, X_3, Z, F$ can be modelled by the BN as shown in Fig.~\ref{bn}, $R_o^{'}\left( {{D_1},{D_2}, {D_3}} \right)  \supseteq  R_o\left( {{D_1},{D_2}, {D_3}} \right)$, and hence  $R_o^{'}\left( {{D_1},{D_2}, {D_3}} \right)  \supseteq  R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right)$ where $R_o^{'}\left( {{D_1},{D_2}, {D_3}} \right)$ is the set of all rate triples $(R_1,R_2,R_3)$ such that there exists a triple $(W_1,W_2,W_3)$ of discrete random variables with $p\left( {{w_1}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_1}|{x_1}} \right)$, $p\left( {{w_2}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_2}|{x_2}} \right)$ and $p\left( {{w_3}|{x_1},{x_2},{x_3},z,f} \right) = p\left( {{w_3}|{x_3}} \right)$ for which the following conditions are satisfied

\begin{equation}
\begin{aligned}
  {R_1} &\geqslant I\left( {{X_1};{W_1}} \right) - I\left( {{W_1};Z,F} \right) \hfill \\
  {R_2} &\geqslant I\left( {{X_2};{W_2}} \right) - I\left( {{W_2};Z,F} \right) \hfill \\
  {R_3} &\geqslant I\left( {{X_3};{W_3}} \right) - I\left( {{W_3};Z,F} \right),
\end{aligned}
\label{outer bound}
\end{equation}
and for which there exist decoding functions ${g_1}\left(  \cdot  \right)$, ${g_2}\left(  \cdot  \right)$ and ${g_3}\left(  \cdot  \right)$ such that
\begin{equation}
\begin{aligned}
E{d_1}({X_1},{g_1(W_1,W_2,W_3,Z,F)}) \leqslant {D_1},\\
E{d_2}({X_2},{g_2(W_2,W_1,W_3,Z,F)}) \leqslant {D_2},\\
E{d_3}({X_3},{g_3(W_3,W_1,W_2,Z,F)}) \leqslant {D_3},
\end{aligned}
\label{constrains}
\end{equation}
\emph{Proof.} First, we can enlarge the region $R_o\left( {{D_1},{D_2}, {D_3}} \right)$ by omitting the sum rate bound in \eqref{theorem3}. Then, the side rate bounds in \eqref{theorem3} can be relaxed as
\begin{equation}
\begin{footnotesize}
\begin{aligned}
{R_1} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right) \\& \geqslant I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right) +I\left( {{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F,X_1} \right) 
\\& \geqslant I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right),
\end{aligned} 
\end{footnotesize}
\label{proof3}
\end{equation}
where $I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right)$ can be written as
\begin{equation}
\begin{footnotesize}
\begin{aligned}
I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right) &= I\left( {{X_1};{W_1},{W_2},{W_3}|Z,F} \right)\\&-I\left( {{X_1};{W_2},{W_3}|Z,F} \right).
\end{aligned} 
\end{footnotesize}
\label{proof4}
\end{equation}
According to the conditional dependence relations as shown Fig.~\ref{bn}, we have $I\left( {{X_1};{W_2},{W_3}|Z,F} \right)=0$, and the term in the right hand side of \eqref{proof4} can be written as
\begin{equation}
\begin{footnotesize}
\begin{aligned}
I\left( {{X_1};{W_1},{W_2},{W_3}|Z,F} \right) &= I\left( {{X_1};{W_1}|Z,F} \right) + I\left( {{X_1};{W_2},{W_3}|Z,F,{W_1}} \right)
\end{aligned} 
\end{footnotesize}
\end{equation}
By the Markov chain $Z, F - X_1 - W_1$, \eqref{proof3} can be written as
\begin{equation}
\begin{aligned}
  {R_1} &\geqslant I\left( {{X_1};{W_1}} \right) - I\left( {{W_1};Z,F} \right).
\end{aligned}
\label{achieve region}
\end{equation}
The same derivation can be applied to $R_2$ and $R_3$, this proves the corollary 5.


\textbf{Theorem 6:} If the joint distribution of $X_1, X_2, X_3, Z, F$ can be modelled by the BN as shown in Fig.~\ref{bn}
\begin{equation}
\begin{footnotesize}
\begin{aligned}
R_a\left( {{D_1},{D_2}, {D_3}} \right) = R_o\left( {{D_1},{D_2}, {D_3}} \right)  =  R_{{X_1},{X_2},{X_3}|Z,F}^{WZ}\left( {{D_1},{D_2}, {D_3}} \right).
\end{aligned}
\label{constrains}
\end{footnotesize}
\end{equation}

\emph{Proof.} We note that the only difference between $R_a\left( {{D_1},{D_2}, {D_3}} \right)$ and $R_o\left( {{D_1},{D_2}, {D_3}} \right)$ is the degrees of freedom when choosing the auxiliary random variables $(W_1, W_2, W_3)$, and all of the mutual information functions in \eqref{achieve region} and \eqref{outer bound} only depend on the marginal distribution $(X_1, W_1, Z, F)$, $(X_2, W_2, Z, F)$ and $(X_3, W_3, Z, F)$. Randomly choose a certain rate triple $(R_1, R_2, R_3)$ with a auxiliary random variable triple $(W_1, W_2, W_3)$ meeting the conditions of Corollary 5, the corresponding joint distribution can be written as 
\begin{equation}
\begin{aligned}
 &p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) \\&= p\left( {w_1},{w_2},{w_3}|{x_1},{x_2},{x_3}\right)p\left( {{x_1}|{z}} \right)p\left( {{x_2}|{z}} \right)p\left( {{x_3}|f} \right) p\left( {{z},f} \right).
\end{aligned}
\label{achieve region}
\end{equation}
Then we construct the auxiliary random variables $(W_1^{'}, W_2^{'}, W_3^{'})$ such that
\begin{equation}
\begin{footnotesize}
\begin{aligned}
{p_{W_1^{'}|{X_1}}}\left( {{w_1}|{s_1}} \right) = \sum\limits_{{w_2},{s_2},{w_3},{s_3}} {p\left( {{w_1},{w_2},{w_3}|{s_1},{s_2},{s_3}} \right)} p\left( {{s_2},{s_3}|{s_1}} \right)\\
{p_{W_2^{'}|{X_2}}}\left( {{w_2}|{s_2}} \right) = \sum\limits_{{w_1},{s_1},{w_3},{s_3}} {p\left( {{w_1},{w_2},{w_3}|{s_1},{s_2},{s_3}} \right)} p\left( {{s_1},{s_3}|{s_2}} \right)\\
{p_{W_3^{'}|{X_3}}}\left( {{w_3}|{s_3}} \right) = \sum\limits_{{w_1},{s_1},{w_2},{s_2}} {p\left( {{w_1},{w_2},{w_3}|{s_1},{s_2},{s_3}} \right)} p\left( {{s_1},{s_2}|{s_3}} \right).
\end{aligned}
\end{footnotesize}
\end{equation}
The joint distribution
\begin{equation}
\begin{footnotesize}
\begin{aligned}
&p\left( {{w_1^{'}},{w_2^{'}},{w_3^{'}},{x_1},{x_2},{x_3},z,f} \right) \\&= p\left( {w_1^{'}}|{x_1}\right)p\left( {w_2^{'}}|{x_2}\right)p\left( {w_3^{'}}|{x_3}\right)p\left( {{x_1}|{z}} \right)p\left( {{x_2}|{z}} \right)p\left( {{x_3}|f} \right) p\left( {{z},f} \right)
\end{aligned}
\end{footnotesize}
\end{equation}
has the same marginal distributions on $(X_1, W_1, Z, F)$, $(X_2, W_2, Z, F)$ and $(X_3, W_3, Z, F)$. Therefore, the additional degree of freedom for choosing the auxiliary random variables $(W_1, W_2, W_3)$ in Corollary 5 can not lower the value of rate-distortion functions. This proves the Theorem 6.


\section{Conclusion}
A variant rate distortion problem  was studied in this paper. First, we derived an achievable rate-distortion region of this problem, and
subsequently, we derived a general outer bound of the rate-distortion region. Finally, we proved that the two regions coincide and obtained a conclusive rate-distortion function under the scenario as shown in Fig.~\ref{bn}

\section*{Appendix A}

\emph{Proof.} Fix $p\left( {{w_1}|{x_1}} \right)$, $p\left( {{w_2}|{x_2}} \right)$ and $p\left( {{w_3}|{x_3}} \right)$ as well as $g_1(W_1,W_2,W_3,Z,F)$, $g_2(W_2,W_1,W_3,Z,F)$ and $g_3(W_3,W_1,W_2,Z,F)$. Calculate $p\left( {{w_1}} \right) = \sum\nolimits_{{x_1}}{p\left( {{x_1}} \right)}p\left( {{w_1}|{x_1}} \right)$,$p\left( {{w_2}} \right) = \sum\nolimits_{{x_2}}{p\left( {{x_2}} \right)}p\left( {{w_2}|{x_2}} \right)$ and $p\left( {{w_3}} \right) = \sum\nolimits_{{x_3}}{p\left( {{x_3}} \right)}p\left( {{w_3}|{x_3}} \right)$.

\emph{Generation of codebooks:}

Generate ${2^{nR_1^{{{'}}}}}$ i.i.d codewords ${{\mathbf{w}}_{\mathbf{1}}}^n\left( {{s_1}} \right) \sim \prod\nolimits_{i = 1}^n {p\left( {{w_{1,i}}} \right)} $, and index them by ${s_1} \in \left\{ {1,2,...,{2^{nR_1^{{'}}}}} \right\}$.

Generate ${2^{nR_2^{{'}}}}$ i.i.d codewords ${{\mathbf{w}}_{\mathbf{2}}}^n\left( {{s_2}} \right) \sim \prod\nolimits_{i = 1}^n {p\left( {{w_{2,i}}} \right)} $, and index them by ${s_2} \in \left\{ {1,2,...,{2^{nR_2^{{'}}}}} \right\}$.

Generate ${2^{nR_3^{{'}}}}$ i.i.d codewords ${{\mathbf{w}}_{\mathbf{3}}}^n\left( {{s_3}} \right) \sim \prod\nolimits_{i = 1}^n {p\left( {{w_{3,i}}} \right)} $, and index them by ${s_3} \in \left\{ {1,2,...,{2^{nR_3^{{'}}}}} \right\}$.

Provide ${2^{nR_1}}$  random bins with indices ${t_1} \in \left\{ {1,2,...,{2^{nR_1}}} \right\}$. Randomly assign the codewords ${{\mathbf{w}}_{\mathbf{1}}}^n\left( {{s_1}} \right)$ to one of ${2^{nR_1}}$ bins using a uniform distribution. Let $ B_1(t_1) $ denote the set of codeword indices $s_1$ assigned to bin index $t_1$.

Provide ${2^{nR_2}}$  random bins with indices ${t_2} \in \left\{ {1,2,...,{2^{nR_2}}} \right\}$. Randomly assign the codewords ${{\mathbf{w}}_{\mathbf{2}}}^n\left( {{s_2}} \right)$ to one of ${2^{nR_2}}$ bins using a uniform distribution. Let $ B_2(t_2) $ denote the set of codeword indices $s_2$ assigned to bin index $t_2$.

Provide ${2^{nR_3}}$  random bins with indices ${t_3} \in \left\{ {1,2,...,{2^{nR_3}}} \right\}$. Randomly assign the codewords ${{\mathbf{w}}_{\mathbf{3}}}^n\left( {{s_3}} \right)$ to one of ${2^{nR_3}}$ bins using a uniform distribution. Let $ B_3(t_3) $ denote the set of codeword indices $s_3$ assigned to bin index $t_3$.

\emph{Encoding:} Given a source sequence $X_1^{n}$, the encoder looks for a codeword $W_1^n(s_1)$ such that $\left( {{X_1^n},W_1^n\left( {{s_1}} \right)} \right) \in A_\epsilon^{*\left( n \right)}$. The encoder sends the index of the bin $t_1$ in which $s_1$ belongs.

Given a source sequence $X_2^{n}$, the encoder looks for a codeword $W_2^n(s_2)$ such that $\left( {{X_2^n},W_2^n\left( {{s_2}} \right)} \right) \in A_\epsilon^{*\left( n \right)}$. The encoder sends the index of the bin $t_2$ in which $s_2$ belongs.

Given a source sequence $X_3^{n}$, the encoder looks for a codeword $W_3^n(s_3)$ such that $\left( {{X_3^n},W_3^n\left( {{s_3}} \right)} \right) \in A_\epsilon^{*\left( n \right)}$. The encoder sends the index of the bin $t_3$ in which $s_3$ belongs.

\emph{Decoding:} The decoder looks for a triple $(W_1^n(s_1),W_2^n(s_2),W_3^n(s_3))$ such that $s_1 \in B_1(t_1) $,  $s_2 \in B_2(t_2) $,  $s_3 \in B_3(t_3) $, and $(W_1^n(s_1),W_2^n(s_2),W_3^n(s_3),Z^n,F^n) \in A_\epsilon^{*\left( n \right)}$. If the decoder finds a unique $s_1,s_2,s_3$, he then calculates $\hat X_1^n,\hat X_2^n,\hat X_3^n$

\emph{Analysis of the probability of error:}

1. The encoders do not find the codewords $W_1^n(s_1)$, $W_2^n(s_2)$, $W_3^n(s_3)$ such that $(X_1^n,W_1^n(s_1)) \in A_\epsilon^{*\left( n \right)}$, $(X_2^n,W_2^n(s_2)) \in A_\epsilon^{*\left( n \right)}$, $(X_3^n,W_1^n(s_3)) \in A_\epsilon^{*\left( n \right)}$. The probability of this event is small if
\begin{equation}
\begin{aligned}
  R_1^{'} > I\left( {{X_1},{W_1}} \right) \hfill \\
  R_2^{'} > I\left( {{X_2},{W_2}} \right) \hfill \\
  R_3^{'} > I\left( {{X_3},{W_3}} \right) \hfill \\ 
\end{aligned}
\label{error1}
\end{equation}

2. The pair of sequences  $(X_1^n,W_1^n(s_1)) \in A_\epsilon^{*\left( n \right)}$, $(X_2^n,W_2^n(s_2)) \in A_\epsilon^{*\left( n \right)}$, $(X_3^n,W_1^n(s_3)) \in A_\epsilon^{*\left( n \right)}$ but the codewords $\{W_1^n(s_1), W_2^n(s_2), W_3^n(s_3)\}$ are not jointly typical with the side information sequences $\{Z^n, F^n\}$, i.e., $(W_1^n(s_1), W_2^n(s_2), W_3^n(s_3), $ $ Z^n, F^n) \notin  A_\epsilon^{*\left( n \right)}$. We have assume that 
\begin{equation}
\begin{aligned}
&p\left( {{w_1},{w_2},{w_3},{x_1},{x_2},{x_3},z,f} \right) \\&= p\left( {{w_1}|{x_1}} \right)p\left( {{w_2}|{x_2}} \right)p\left( {{w_3}|{x_3}} \right)p\left( {{x_1},{x_2},{x_3},z,f} \right).
\end{aligned}
\label{error2}
\end{equation}
Hence, by the Markov lemma, the probability of this event goes to zero if n is large enough.

3. There exists an alternative choice of three codewords that is jointly typical with the side information sequences.
Denote the correct codeword indices by $s_1$, $s_2$ and $s_3$. We first consider the situation that the first codeword index is in error while the rest indices are correct. The probability that a randomly chosen $W_1^n(s^{'}_1)$ is jointly typical with $(W_2^n(s_2),W_3^n(s_3),Z^n,F^n)$ can be bounded as
\begin{equation}
\begin{aligned}
&\Pr \left\{ {\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {{s_2}} \right),W_3^n\left( {{s_3}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)}} \right\}\\& \leqslant {2^{ - n\left( {\left( {{W_1};{W_2},{W_3},Z,F} \right) - 3\epsilon} \right)}}.
\end{aligned}
\label{error3}
\end{equation}
The decoder may confuse with any one of the codeword  ${{\mathbf{w}}_{\mathbf{1}}}^n\left( {{s^{'}_1}} \right)$ that have bin index $t_1$. Hence the error probability is
\begin{equation}
\begin{footnotesize}
\begin{aligned}
  &\Pr \left\{ \exists s_1^{'} \in {B_1}\left( {{t_1}} \right),s_1^{'} \ne {s_1}:\right.\\
  &\left.\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {{s_2}} \right),W_3^n\left( {{s_3}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)} \right\} \hfill \\&
   \leqslant \sum\limits_{s_1^{'} \ne {s_1},\atop s_1^{'} \in {B_1}\left( {{t_1}} \right)} {\Pr \left\{ {\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {{s_2}} \right),W_3^n\left( {{s_3}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)}} \right\}}  \hfill \\
   &\leqslant {2^{n\left( {{R_1} - R_1^{'}} \right)}}{2^{ - n\left( {I\left( {{W_1};{W_2},{W_3},Z,F} \right) - 3\epsilon} \right)}}.
\end{aligned}
\label{error4}
\end{footnotesize}
\end{equation}
The same derivation applies to the situations where the second or the third codeword is in error.

We then consider the case where both the first codeword index and the second codeword index are in error. The probability that the randomly chosen $W_1^n(s^{'}_1)$ and $W_2^n(s^{'}_2)$ are jointly typical with $(W_3^n(s_3),Z^n,F^n)$ can be bounded as
\begin{equation}
\begin{footnotesize}
\begin{aligned}
  &\Pr \left\{ {\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),W_2^n\left( {{s_3}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)}} \right\} \hfill \\&
   = \sum\limits_{\left( {{W_1},{W_2},{W_3},Z,F} \right) \in A_\epsilon^{*\left( n \right)}} {p\left( {w_1^n} \right)p\left( {w_2^n} \right)p\left( {w_3^n,{z^n},{f^n}} \right)}  \hfill \\&
   \leqslant {2^{n\left( {H\left( {{W_1},{W_2},{W_3},Z,F} \right) + \epsilon} \right)}}{2^{ - n\left( {H\left( {{W_1}} \right) - \epsilon} \right)}}\\
   &\times {2^{ - n\left( {H\left( {{W_2}} \right) - \epsilon} \right)}}{2^{ - n\left( {H\left( {{W_3},Z,F} \right) - \epsilon} \right)}} \hfill \\
   &= 2^n\left( H\left( {{W_3},Z,F} \right) + H\left( {{W_2}|{W_3},Z,F} \right) \right.\\
   &+ H\left( {{W_1}|{W_2},{W_3},Z,F} \right) - H\left( {{W_1}} \right) \\
  &\left. - H\left( {{W_2}} \right) - H\left( {{W_3},Z,F} \right) + 4\epsilon \right) \hfill \\&
   = {2^{ - n\left( {I\left( {{W_1};{W_2},{W_3},Z,F} \right) + I\left( {{W_2};{W_3},Z,F} \right) - 4\epsilon} \right)}} \hfill \\&
   = {2^{ - n\left( {I\left( {{W_1};{W_2},{W_3},Z,F} \right) + I\left( {{W_2};{W_1},{W_3},Z,F} \right) - I\left( {{W_1};{W_2}|{W_3},Z,F} \right) - 4\epsilon} \right)}} \hfill.
\end{aligned}
\label{error5}
\end{footnotesize}
\end{equation}
Hence the error probability is
\begin{equation}
\begin{aligned}
  &\Pr \left\{ \exists s_1^{'} \in {B_1}\left( {{t_1}} \right),s_1^{'} \ne {s_1},\exists s_2^{'} \in {B_2}\left( {{t_2}} \right),s_2^{'} \ne {s_2}:\right.\\
  &\left. \left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),W_2^n\left( {{s_3}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)} \right\} \hfill \\
  &\leqslant \sum\limits_{s_1^{'} \ne {s_1}, s_1^{'} \in {B_1}\left( {{t_1}} \right),\atop s_2^{'} \ne {s_2}, s_2^{'} \in {B_2}\left( {{t_2}} \right)} \Pr \left\{ \left( W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),\right.\right.\\ 
  &\left.\left.W_2^n\left( {{s_3}} \right),{Z^n},{F^n} \right)  \in A_\epsilon^{*\left( n \right)} \right\}  \hfill 
  \\&
   \leqslant {2^{n( {{R_1} - R_1^{'} + {R_2} - R_2^{'}} )}}\\
   &\times 2^{ - n\left( {I\left( {{W_1};{W_2},{W_3},Z,F} \right) + I\left( {{W_2};{W_1},{W_3},Z,F} \right)  - I\left( {{W_1};{W_2}|{W_3},Z,F} \right) - 4\epsilon} \right)} \hfill .
\end{aligned}
\label{error6}
\end{equation}

We then consider the case where all the  codeword indices  are in error. The probability that the randomly chosen $W_1^n(s^{'}_1)$, $W_2^n(s^{'}_2)$ and $W_3^n(s^{'}_3)$ are jointly typical with $(Z^n,F^n)$ can be bounded as

\begin{equation}
\begin{aligned}
  &\Pr \left\{ {\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),W_2^n\left( {s_3^{'}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)}} \right\} \hfill \\&
   = \sum\limits_{\left( {{W_1},{W_2},{W_3},Z,F} \right) \in A_\epsilon^{*\left( n \right)}} {p\left( {w_1^n} \right)p\left( {w_2^n} \right)p\left( {w_3^n} \right)p\left( {{z^n},{f^n}} \right)}  \hfill \\&
   \leqslant {2^{n\left( {H\left( {{W_1},{W_2},{W_3},Z,F} \right) + \epsilon} \right)}}{2^{ - n\left( {H\left( {{W_1}} \right) - \epsilon} \right)}}{2^{ - n\left( {H\left( {{W_2}} \right) - \epsilon} \right)}}\\
   &\times {2^{ - n\left( {H\left( {{W_3}} \right) - \epsilon} \right)}}{2^{ - n\left( {H\left( {Z,F} \right) - \epsilon} \right)}} \hfill \\
   % &= {2^{n\left( {H\left( {{W_3},Z,F} \right) + H\left( {{W_2}|{W_3},Z,F} \right) + H\left( {{W_1}|{W_2},{W_3},Z,F} \right) - H\left( {{W_1}} \right) - H\left( {{W_2}} \right) - H\left( {{W_3}} \right) - H\left( {Z,F} \right) + 5\epsilon} \right)}} \hfill \\
   &= {2^{ - n\left( {I\left( {{W_3};Z,F} \right) + I\left( {{W_2};{W_3},Z,F} \right) + I\left( {{W_1};{W_2},{W_3},Z,F} \right) - 5\epsilon} \right)}} \hfill \\&
   = 2^{ - n\left( I\left( {{W_1};{W_2},{W_3},Z,F} \right) + I\left( {{W_2};{W_1},{W_3},Z,F} \right)\right)}\\
   &\times 2^{ -n\left( I\left( {{W_3};{W_1},{W_2},Z,F} \right) - I\left( {{W_1};{W_2}|{W_3},Z,F} \right) - I\left( {{W_1},{W_2};{W_3}|Z,F} \right) - 5\epsilon \right)} \hfill.
\end{aligned}
\label{error7}
\end{equation}
Hence the error probability is
\begin{equation}
\begin{footnotesize}
\begin{aligned}
  &\Pr \left\{ \exists s_1^{'} \in {B_1}\left( {{t_1}} \right),s_1^{'} \ne {s_1},\exists s_2^{'} \in {B_2}\left( {{t_2}} \right),s_2^{'} \ne {s_2},\right.\\
  &\left.\exists s_3^{'} \in {B_3}\left( {{t_3}} \right),s_3^{'} \ne {s_3}:\right.\\
  &\left.\left( {W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),W_2^n\left( {s_3^{'}} \right),{Z^n},{F^n}} \right) \in A_\epsilon^{*\left( n \right)}\right\} \hfill \\&
   \leqslant \sum\limits_{s_1^{'} \ne {s_1},s_1^{'} \in {B_1} \left( {{t_1}} \right), s_2^{'} \ne {s_2}, \atop s_2^{'} \in {B_2}\left( {{t_2}} \right),s_3^{'} \ne {s_3},s_3^{'} \in {B_3}\left( {{t_3}} \right)} \Pr \left\{ \left( W_1^n\left( {s_1^{'}} \right),W_2^n\left( {s_2^{'}} \right),\right.\right.\\
   &\left.\left. W_2^n\left( {{s_3}} \right),{Z^n},{F^n} \right) \in A_\epsilon^{*\left( n \right)} \right\}  \hfill \\&
   \leqslant {2^{n\left( {{R_1} - R_1^{'} + {R_2} - R_2^{'} + {R_3} - R_3^{'}} \right)}}\\
   &\times {2^{ - n\left( {I\left( {{W_1};{W_2},{W_3},Z,F} \right) + I\left( {{W_2};{W_1},{W_3},Z,F} \right) + I\left( {{W_3};{W_1},{W_2},Z,F} \right)}\right)}}\\
   &\times {2^{-n\left({- I\left( {{W_1};{W_2}|{W_3},Z,F} \right) - I\left( {{W_1},{W_2};{W_3}|Z,F} \right) - 5\epsilon} \right)}} \hfill .
\end{aligned}
\label{error8}
\end{footnotesize}
\end{equation}
Therefore, we have 
\begin{equation}
\begin{footnotesize}
\begin{aligned}
  &R_1^{'} - {R_1} \\&\leqslant I\left( {{W_1};{W_2},{W_3},Z,F} \right) \hfill \\
 & R_1^{'} - {R_1} + R_2^{'} - {R_2} \\&\leqslant I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\& + I\left( {{W_2};{W_1},{W_3},Z,F} \right) - I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \hfill \\
 & R_1^{'} - {R_1} + R_2^{'} - {R_2} + R_3^{'} - {R_3} \\&\leqslant I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\&+ I\left( {{W_2};{W_1},{W_3},Z,F} \right) + I\left( {{W_3};{W_1},{W_2},Z,F} \right) \\&- I\left( {{W_1};{W_2}|{W_3},Z,F} \right) - I\left( {{W_1},{W_2};{W_3}|Z,F} \right).
\end{aligned}
\label{error8}
\end{footnotesize}
\end{equation}

(\ref{achieve region}) can be obtained by combining (\ref{error1}) and (\ref{error8}).

\section*{Appendix B}
\begin{equation}
\begin{footnotesize}
\begin{aligned}
nR_1\geq& H(T_1)\\
\geq & H(T_1|T_2, T_3, Z^n, F^n)\\
\geq & H(T_1|T_2, T_3, Z^n, F^n) - H(T_1|T_2, T_3,Z^n, F^n, X_1^n, X_2^n, X^n_3)\\
= & I(X_1^n, X_2^n, X_3^n; T_1|T_2, T_3, Z^n, F^n)\\
=& \sum\limits_{i=1}^n I(X_{1i}, X_{2i}, X_{3i}; T_1 | T_2, T_3, Z^n, F^n, X_{11}^{i-1}, X_{21}^{i-1}, X_{31}^{i-1})\\
=&\sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i}| T_2, T_3, Z^n, F^n, X_{11}^{i-1}, X_{21}^{i-1}, X_{31}^{i-1}) \\
&- H(X_{1i}, X_{2i}, X_{3i}; T_1 | T_2, T_3, Z^n, F^n, X_{11}^{i-1}, X_{21}^{i-1}, X_{31}^{i-1})\\
=& \sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i} | W_{2i}, W_{3i}, Z_i, F_i)\\
&- H(X_{1i}, X_{2i}, X_{3i} | W_{1i}, W_{2i}, W_{3i}, Z_i, F_i)\\
=& \sum\limits_{i=1}^n I(X_{1i}, X_{2i}, X_{3i}; W_{1i} | W_{2i}, W_{3i}, Z_i, F_i),
\end{aligned}
\end{footnotesize}
\end{equation}
where ${W_{1i}} = \left( {{T_1},X_{1,1}^{i - 1},X_{2,1}^{i - 1},X_{3,1}^{i - 1},Z_1^{i - 1},Z_{i + 1}^n,F_1^{i - 1},}\right.$ $\left.{F_{i + 1}^n} \right)$, ${W_{2i}} = \left( {{T_2},X_{1,1}^{i - 1},X_{2,1}^{i - 1},X_{3,1}^{i - 1},Z_1^{i - 1},Z_{i + 1}^n,F_1^{i - 1},}\right.$ $\left.{F_{i + 1}^n} \right),{W_{3i}} = \left( {{T_1},X_{1,1}^{i - 1},X_{2,1}^{i - 1},X_{3,1}^{i - 1},Z_1^{i - 1},Z_{i + 1}^n,F_1^{i - 1},}\right.$ $\left.{F_{i + 1}^n} \right)$.

Then we prove ${R_1} \geqslant I\left( {{X_1};{W_1}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right) = I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right)$
\begin{equation}
\begin{aligned}
    &I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right) \\
    &= I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right) \\
    &+ \underbrace {I\left( {{X_2},{X_3};{W_1}|{X_1},{W_2},{W_3},Z,F} \right)}_0.
\end{aligned}
\end{equation}
For the first term of the right
\begin{equation}
\begin{aligned}
  &I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right) + I\left( {{W_1};{W_2},{W_3},Z,F} \right) \\
  &= I\left( {{W_1};{X_1},{W_2},{W_3},Z,F} \right) \hfill \\
   &= I\left( {{W_1};{X_1}} \right) + \underbrace {I\left( {{W_1}|{X_1};{W_2},{W_3},Z,F} \right)}_0. 
\end{aligned}
\end{equation}
Then we have
\begin{equation}
\begin{aligned}
&I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right) \\
&= I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right) \\
&= I\left( {{W_1};{X_1}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right).
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
{R_1} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1}|{W_2},{W_3},Z,F} \right) \\&= I\left( {{W_1};{X_1}} \right) - I\left( {{W_1};{W_2},{W_3},Z,F} \right)
\end{aligned}
\end{equation}
Similarly, we have
\begin{equation}
\begin{aligned}
{R_2} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F} \right) \\&= I\left( {{W_2};{X_2}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
{R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_3}|{W_1},{W_2},Z,F} \right) \\&= I\left( {{W_3};{X_3}} \right) - I\left( {{W_3};{W_1},{W_2},Z,F} \right)
\end{aligned}
\end{equation}


\begin{equation}
\begin{aligned}
&n(R_1+R_2)\\
\geq & H(T_1, T_2)\\
\geq & H(T_1, T_2 | Z^n, F^n, T_3)\\
\geq & H(T_1, T_2| Z^n, F^n, T_3) - \\
&H(T_1, T_2| Z^n, F^n, T_3, X_1^n, X_2^n, X_3^n)\\
 = & I(T_1, T_2; X_1^n, X_2^n, X_3^n | Z^n, F^n, T_3)\\
 =& \sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i} | Z^n, F^n, T_3, X_1^{i-1}, X_2^{i-1}, X_3^{i-1}) \\
 &- H(X_{1i}, X_{2i}, X_{3i} | T_1, T_2, X_{11}^{i-1}, X_{21}^{i-1}, X_{31}^{i-1}, Z^n, F^n, T_3)\\
 =& \sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i} | Z^n, F^n, W_{3i}) \\
 &- H(X_{1i}, X_{2i}, X_{3i} | W_{1i}, W_{2i}, W_{3i}, Z_i, F_i) \\ 
=& I(X_1, X_2, X_3; W_1, W_2| Z, F, W_3)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
  &I\left( {{X_1},{X_2},{X_3};{W_1},{W_2}|{W_3},Z,F} \right)\\
  &= I\left( {{X_1};{W_1},{W_2}|{W_3},Z,F} \right) \\
  &+ I\left( {{X_2},{X_3};{W_1},{W_2}|{W_3},Z,F,{X_1}} \right) \hfill \\&
   = I\left( {{X_1};{W_2}|{W_3},Z,F} \right) + \underbrace {I\left( {{X_1};{W_1}|{W_2},{W_3},Z,F} \right)}_{{R_1}} \\
   &+ \underbrace {I\left( {{X_2},{X_3};{W_1}|{W_3},Z,F,{X_1}} \right)}_0 \\&+ I\left( {{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F,{X_1}} \right) \hfill 
\end{aligned}
\end{equation}
For the last term in the right hand side
\begin{equation}
\begin{aligned}
  &I\left( {{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F,{X_1}} \right) + I\left( {{X_1};{W_2}|{W_1},{W_3},Z,F} \right)\\
  &= I\left( {{X_1},{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F} \right) \hfill \\&
   = I\left( {{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F} \right) \\
   &+ \underbrace {I\left( {{X_1};{W_2}|{W_1},{W_3},Z,F,{X_2},{X_3}} \right)}_0 \hfill \\&
   = \underbrace {I\left( {{X_2};{W_2}|{W_1},{W_3},Z,F} \right)}_{{R_2}} \\
   &+ \underbrace {I\left( {{X_1},{X_3};{W_2}|{W_1},{W_3},Z,F,{X_2}} \right)}_0 \hfill
\end{aligned}
\end{equation}
Then we have
\begin{equation}
\begin{aligned}
&I\left( {{X_2},{X_3};{W_2}|{W_1},{W_3},Z,F,{X_1}} \right) \\
=& \underbrace {I\left( {{X_2};{W_2}|{W_1},{W_3},Z,F} \right)}_{{R_2}} - I\left( {{X_1};{W_2}|{W_1},{W_3},Z,F} \right)
\end{aligned}
\end{equation}
For the last term in the right hand side
\begin{equation}
\begin{aligned}
   &I\left( {{X_1};{W_2}|{W_1},{W_3},Z,F} \right) \hfill + I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \\
   &= I\left( {{X_1},{W_1};{W_2}|{W_3},Z,F} \right) \hfill \\
   &= I\left( {{X_1};{W_2}|{W_3},Z,F} \right) + \underbrace {I\left( {{W_1};{W_2}|{X_1},{W_1},{W_3},Z,F} \right)}_0 \hfill \\ 
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
&I\left( {{X_1};{W_2}|{W_1},{W_3},Z,F} \right)\\
=& I\left( {{X_1};{W_2}|{W_3},Z,F} \right) - I\left( {{W_1};{W_2}|{W_3},Z,F} \right)
\end{aligned}
\end{equation}
Then we have
\begin{equation}
\begin{aligned}
{R_1} + {R_2} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1},{W_2}|{W_3},Z,F} \right) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) \\
&- I\left( {{W_1};{W_2},{W_3},Z,F} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\
&+ I\left( {{W_1};{W_2}|{W_3},Z,F} \right)
\end{aligned}
\end{equation}
Similarly, we have
\begin{equation}
\begin{aligned}
{R_1} + {R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_1},{W_3}|{W_2},Z,F} \right) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_3};{W_3}} \right)\\
&- I\left( {{W_1};{W_2},{W_3},Z,F} \right) - I\left( {{W_3};{W_1},{W_2},Z,F} \right) \\
&+ I\left( {{W_1};{W_3}|{W_2},Z,F} \right)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
{R_2} + {R_3} &\geqslant I\left( {{X_1},{X_2},{X_3};{W_2},{W_3}|{W_1},Z,F} \right) \\&= I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right)\\
&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_2};{W_3}|{W_1},Z,F} \right)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
&n(R_1 + R_2 + R_3)\\
\geq & H(T_1, T_2, T_3)\\
\geq & H(T_1, T_2, T_3 | Z^n, F^n) \\ 
\geq & H(T_1, T_2, T_3|Z^n, F^n) - H(T_1, T_2, T_3 | Z^n, F^n, X_1, X_2, X_3) \\ 
= & I(T_1, T_2, T_3 ; X_1^n, X_2^n, X_3^n | Z^n, F^n) \\ 
=& \sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i} | Z^n, F^n, X_1^{i-1}, X_2^{i-1}, X_3^{i-1}) \\
&- H(X_{1i}, X_{2i}, X_{3i} | T_1, T_2, T_3, X_{11}^{i-1}, X_{21}^{i-1}, X_{31}^{i-1}, Z, F)\\
=& \sum\limits_{i=1}^n H(X_{1i}, X_{2i}, X_{3i} | Z, F, X_1^{i-1}, X_2^{i-1}, X_3^{i-1}) \\
&- H(X_{1i}, X_{2i}, X_{3i} | W_1, W_2, W_3, Z, F)\\
=& \sum I(X_1, X_2, X_3; W_1, W_2, W_3| Z, F)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
&I\left( {{X_1},{X_2},{X_3};{W_1},{W_2},{W_3}|Z,F} \right)  \\
&= I\left( {{X_1};{W_1},{W_2},{W_3}|Z,F} \right) + I\left( {{X_2};{W_1},{W_2},{W_3}|Z,F,{X_1}} \right)\\
&+ I\left( {{X_3};{W_1},{W_2},{W_3}|Z,F,{X_1},{X_2}} \right) \hfill \\ 
\end{aligned}
\label{r123}
\end{equation}
For the first term in the right hand side
\begin{equation}
\begin{aligned}
&I\left( {{X_1};{W_1},{W_2},{W_3}|Z,F} \right) \\
=& I\left( {{X_1};{W_3}|Z,F} \right) + I\left( {{X_1};{W_2}|Z,F,{W_3}} \right)\\
&+ \underbrace {I\left( {{X_1};{W_1}|Z,F,{W_2},{W_3}} \right)}_{{R_1}}
\end{aligned}
\end{equation}
 For the second term in the right hand side of (\ref{r123})
\begin{equation}
\begin{aligned}
&I\left( {{X_2};{W_1},{W_2},{W_3}|Z,F,{X_1}} \right)\\
=& \underbrace {I\left( {{X_2};{W_1}|Z,F,{X_1}} \right)}_0 \\
&+ \underbrace {I\left( {{X_2};{W_3}|Z,F,{X_1},{W_1}} \right)}_0 + I\left( {{X_2};{W_2}|Z,F,{X_1},{W_1},{W_3}} \right)
\end{aligned}
\end{equation}
For the last term in the right hand side
\begin{equation}
\begin{aligned}
  &I\left( {{X_2};{W_2}|Z,F,{X_1},{W_1},{W_3}} \right) + I\left( {{X_1};{W_2}|Z,F,{W_1},{W_3}} \right)\\
  =& I\left( {{X_1},{X_2};{W_2}|Z,F,{W_1},{W_3}} \right) \hfill \\
   =& \underbrace {I\left( {{X_1},{X_2};{W_2}|Z,F,{W_1},{W_3}} \right)}_{{R_2}} \\
   &+ \underbrace {I\left( {{X_1},{X_2};{W_2}|Z,F,{W_1},{W_3}} \right)}_0 .
\end{aligned}
\end{equation}
Then we have
\begin{equation}
\begin{aligned}
&I\left( {{X_2};{W_2}|Z,F,{X_1},{W_1},{W_3}} \right)\\
=& \underbrace {I\left( {{X_1},{X_2};{W_2}|Z,F,{W_1},{W_3}} \right)}_{{R_2}} - I\left( {{X_1};{W_2}|Z,F,{W_1},{W_3}} \right)
\end{aligned}
\end{equation}
For the last term in the right hand side
\begin{equation}
\begin{aligned}
  &I\left( {{X_1};{W_2}|Z,F,{W_1},{W_3}} \right) + I\left( {{W_1};{W_2}|Z,F,{W_3}} \right) \hfill \\
   =& I\left( {{X_1},{W_1};{W_2}|Z,F,{W_3}} \right) \hfill \\
   =& I\left( {{X_1};{W_2}|Z,F,{W_3}} \right) + \underbrace {I\left( {{W_1};{W_2}|Z,F,{W_3},{X_1}} \right)}_0 \hfill \\ 
\end{aligned}
\end{equation}
Then we have
\begin{equation}
\begin{aligned}
  &I\left( {{X_1};{W_2}|Z,F,{W_1},{W_3}} \right)\\
  =& I\left( {{X_1};{W_2}|Z,F,{W_3}} \right) -  I\left( {{W_1};{W_2}|Z,F,{W_3}} \right)\hfill \\ 
\end{aligned}
\end{equation}
For the third term in the right hand side of (\ref{r123})
\begin{equation}
\begin{aligned}
  &I\left( {{X_3};{W_1},{W_2},{W_3}|Z,F,{X_1},{X_2}} \right) \\
  =& \underbrace {I\left( {{X_3};{W_1},{W_2}|Z,F,{X_1},{X_2}} \right)}_0\\
  &+ I\left( {{X_3};{W_3}|Z,F,{X_1},{X_2},{W_1},{W_2}} \right) \hfill 
\end{aligned}
\end{equation}
For the last term in the right hand side

\begin{equation}
\begin{aligned}
  &I\left( {{X_3};{W_3}|Z,F,{X_1},{X_2},{W_1},{W_2}} \right)\\
  &+ I\left( {{X_1},{X_2};{W_3}|Z,F,{W_1},{W_2}} \right)\\
  =& I\left( {{X_1},{X_2},{X_3};{W_3}|Z,F,{W_1},{W_2}} \right) \hfill \\
   =& \underbrace {I\left( {{X_3};{W_3}|Z,F,{W_1},{W_2}} \right)}_{{R_3}} \\
   &+ \underbrace {I\left( {{X_1},{X_2};{W_3}|Z,F,{W_1},{W_2},{X_3}} \right)}_0 \hfill
\end{aligned}
\end{equation}

Then we have
\begin{equation}
\begin{aligned}
&I\left( {{X_3};{W_3}|Z,F,{X_1},{X_2},{W_1},{W_2}} \right)\\
=& \underbrace {I\left( {{X_3};{W_3}|Z,F,{W_1},{W_2}} \right)}_{{R_3}} - I\left( {{X_1},{X_2};{W_3}|Z,F,{W_1},{W_2}} \right)
\end{aligned}
\end{equation}
For the last term in the right hand side


\begin{equation}
\begin{aligned}
&I\left( {{X_1},{X_2};{W_3}|Z,F,{W_1},{W_2}} \right) \\
=& I\left( {{X_1},{X_2},{W_1},{W_2};{W_3}|Z,F} \right) - I\left( {{W_1},{W_2};{W_3}|Z,F} \right)
\end{aligned}
\end{equation}
For the first term in the right hand side 
\begin{equation}
\begin{aligned}
  &I\left( {{X_1},{X_2},{W_1},{W_2};{W_3}|Z,F} \right)\\
  =& I\left( {{X_1};{W_3}|Z,F} \right) + I\left( {{X_2},{W_1},{W_2};{W_3}|Z,F,{X_1}} \right) \hfill \\
   =& I\left( {{X_1};{W_3}|Z,F} \right) + \underbrace {I\left( {{X_2};{W_3}|Z,F,{X_1}} \right)}_0\\
   &+ \underbrace {I\left( {{W_1},{W_2};{W_3}|Z,F,{X_1},{X_2}} \right)}_0 \hfill \\ 
\end{aligned}
\end{equation}

Then we have
\begin{equation}
\begin{aligned}
&{R_1} + {R_2} + {R_3} \\
&\geqslant I(X_1, X_2, X_3; W_1, W_2, W_3| Z, F) \\&= I\left( {{X_1};{W_1}} \right) + I\left( {{X_2};{W_2}} \right) + I\left( {{X_3};{W_3}} \right) \\&- I\left( {{W_1};{W_2},{W_3},Z,F} \right) - I\left( {{W_2};{W_1},{W_3},Z,F} \right) \\&- I\left( {{W_3};{W_1},{W_2},Z,F} \right) + I\left( {{W_1};{W_2}|{W_3},Z,F} \right) \\&+ I\left( {{W_1},{W_2};{W_3}|Z,F} \right),
\end{aligned}
\end{equation}
\begin{comment}

\begin{abstract}

\end{abstract}

\begin{IEEEkeywords}

\end{IEEEkeywords}

\section{Introduction}
This document is a model and instructions for \LaTeX.
Please observe the conference page limits. 

\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.


\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.
\end{comment}

\bibliographystyle{IEEEtran}
\bibliography{ref}

\end{document}

